Human-Planned Robotic Grasp Ranges: Capture and Validation

Leveraging human grasping skills to teach a robot to perform a manipulation task is appealing, but there are several limitations to this approach: time-inefficient data capture procedures, limited generalization of the data to other grasps and objects, and inability to use that data to learn more about how humans perform and evaluate grasps. This paper presents a data capture protocol that partially addresses these deficiencies by asking participants to specify ranges over which a grasp is valid. The protocol is verified both qualitatively through online survey questions (where 95.38% of within-range grasps are identified correctly with the nearest extreme grasp) and quantitatively by showing that there is small variation in grasps ranges from different participants as measured by joint angles, contact points, and position. We demonstrate that these grasp ranges are valid through testing on a physical robot (93.75% of grasps interpolated from grasp ranges are successful).

==> OldText.tex <==
This equipment was used to capture the following:
\begin{itemize}
\item Eye gaze location while grasping objects.
\item Human grasps for different objects.
\item Robotic grasps for different objects.
\item Human defined ranges for all grasps.
\item Grasps classified as "good" and "bad" for each task.
\end{itemize}

[TODO: add image of calibration mark]

The general flow of the study can be seen in Figure \ref{fig:procedure} or in the list below.

\begin{enumerate}
\item Subject enters room and signs consent form.
\item Brief training session with a test object.
\item Study trials explained to subject.
\item Eye tracking calibration performed.
\item Object placed on table, and subject told to use either robot or their own hand first.
\item Pick up task performed.
\item Natural task performed.
\item Eye tracking recording stopped, and re-calibration if needed. 
\item Tasks repeated with hand not used earlier.
\item Eye tracking recording stopped, all other data collection ended.
\item Process repeated with rest of objects as time allows.
\end{enumerate}

The streamlined data collection process uses ROS to integrate and store data feeds from the Barrett hand, the Barrett arm, and the Kinect. RGB and depth images are recorded continuously during the grasping phases along with the robot's arm and hand joint positions when it is being manipulated. When subjects decide on a particular grasp, a small fixed-format annotation is added to the data stream along with a timestamp for future synchronization. The above system is separate from the system collecting video and gaze data from the eye-tracking glasses. The two systems are time synchronized using a short, high-pitched beep emitted by the PC before each trial. Grasps can be flagged during recording of the eye-tracking data to make them easier to find in the video data.



[TODO: describe procedure (recording programs started on machine running ROS, eye tracking calibration. ]

For the latter,
For each object, there is a trial in which subjects indicate good grasps, as well as a trial where subjects indicate bad grasps. The subjects were asked to think out loud as they perform the study to provide insight of what they were thinking while grasping. The setup can be found in Figure \ref{fig:setup}.

In each phase, the subjects were first instructed to grab an object with the intention of picking it up. After indicating their grasps for picking up the object, the subjects were then asked to indicate grasps for performing a natural task with that object. These natural tasks are tasks or actions that are associated with each object, such as throwing a ball, squeezing a trigger, or handing the object to someone.

For each specified grasp, the subject is then asked to provide a range along the object for which that particular grasp can still be applied (e.g. along the side of a box, along a handle). Subjects are also asked if there are any rotational or symmetric ranges for their grasps. In the good grasp trial, these ranges are the areas on the object that the subject believes the grasp would still be successful. In the bad grasp trial this range represents the region that a particular grasp would still be ineffective.

The IRB approved study is set up to be run by two researchers. The data collection can be split up over multiple sessions. The average time for a data collection block was an hour and a half, covering three or four objects. The maximum time used for a subject is capped at two hours due to eye strain generated by the eye tracking glasses, as well as general fatigue from performing the experiment. Before starting the experiment there is a training session that allows the subject to become accustomed to moving the robotic arm and closing the robotic hand around an object.

There are two roles for performing the study, one researcher works mostly with the Ubuntu Linux PC running ROS, and one researcher works with the SMI eye tracking laptop. Both researchers play a role in explaining the study and talking to the subject. 

To collect data evenly for the good and bad trials subjects that we collect data from only once are asked to perform good grasps on two objects first, and then bad grasps with two objects second. Some subjects had multiple sessions, and in this case they performed good grasps in the first session, and bad grasps in the second.



While these images can be used independently of each other to extract features or perform hand tracking, the real benefit shows when combining the data. To do this we produce a point cloud, which is simply a collection of 3 dimensional points with x,y, and z components that also have an RGB color attached to them. This is generated by aligning the depth data frame with the RGB image, and rendering each depth point with the corresponding color from the RGB image [TODO: should use a reference to image alignment for point clouds]. This gives us a 3D model of the scene viewed by the Kinect, which is valuable as it creates a correlation between the color image and our objects by bringing it into 3D, and also creates a context for the depth data.

The streamlined data collection process uses ROS to integrate and store data feeds from the Barrett hand, the Barrett arm, and the Kinect. RGB and depth images are recorded continuously during the grasping phases along with the robot's arm and hand joint positions when it is being manipulated. When subjects decide on a particular grasp, a small fixed-format annotation is added to the data stream along with a timestamp for future synchronization. The above system is separate from the system collecting video and gaze data from the eye-tracking glasses. The two systems are time synchronized using a short, high-pitched beep emitted by the PC before each trial. Grasps can be flagged during recording of the eye-tracking data to make them easier to find in the video data.

\subsubsection{Microsoft Kinect}

The Microsoft Kinect works as a camera and as a depth sensor. This gives us an RGB image as seen in Figure \ref{fig:rgb} and depth data in the form of an image, as seen in Figure \ref{fig:depth}. The depth data is different from a traditional image in that it doesn't represent color, instead it uses each element in the image to represent a distance from the camera. Any values that don't register a depth are left as 0, which includes objects that are too far away, or did not reflect any infrared light. This information can be used to define a 3D shape for objects in the scene.

While these images can be used independently of each other to extract features or perform hand tracking, the real benefit shows when combining the data. To do this we produce a point cloud, which is simply a collection of 3 dimensional points with x,y, and z components that also have an RGB color attached to them. This is generated by aligning the depth data frame with the RGB image, and rendering each depth point with the corresponding color from the RGB image [TODO: should use a reference to image alignment for point clouds]. This gives us a 3D model of the scene viewed by the Kinect, which is valuable as it creates a correlation between the color image and our objects by bringing it into 3D, and also creates a context for the depth data.

An example point cloud can be seen in Figure [TODO], and a simulation generated from this data can be seen in Figure [TODO].


----------------------
The arm and Kinect data were timestamped and synced using a linux program called chrony running within ROS. This syncs the system time of two different computers over a network. The only data that still needs to by synced is the eye tracking data. The recording program runs on a separate Windows laptop, and cannot sync with the linux based machines.

To address this issue we use an audio cue of a 5 KhZ beep to mark a common point in both data streams. This beep is emitted at the beginning of data recording from a speaker on the ROS desktop machine. The microphone on the eye tracking glasses records audio as well, and provides a consistent stream of audio to analyze.

As seen in Figure \ref{fig:fft} we can detect this point in time by looking for a spike in the 5 KhZ frequency. To accomplish this we use a windowed Fast Fourier Transform (FFT), which represents the signal over time as a distribution of frequencies. The response in 5 KhZ can be used for beep detection as it represents a large increase in the 5 KhZ frequency. While there is some noise in this response, the spike is generally easy to identify due to the increased volume of the beep.

The function works over the whole audio stream in 100 ms windows. The detection looks for a slope increase of a positive parameter, and returns the time value for the first window to satisfy this. We settled on using a parameter value of 1, but this could change depending on distance from the speaker, and other noise.

Due to the choice of 100 ms windows, the error in this detection could be up to 50 ms given a good choice in slope threshold. To improve, the process could be run iteratively on the resulting window. This would identify the beep at a finer detail of time, and better align the data.

After this point is detected gaze data for a given video time can be synced to data at the appropriate time from the ROS data. Also included in this analysis tool is the parsing of an annotation file produced during the study. The annotation file contains notes about the experiment, such as when sets of grasps begin, or moments when a grasp range is specified. 

The program lets the user select both the annotation file, and the corresponding eye tracking video. The annotations are then output in times relative to the eye tracking data for alignment. This can be seen in Figure \ref{fig:annotation}.


After this point is detected gaze data for a given video time can be synced to data at the appropriate time from the ROS data. Also included in this analysis tool is the parsing of an annotation file produced during the study. The annotation file contains notes about the experiment, such as when sets of grasps begin, or moments when a grasp range is specified. 

The program lets the user select both the annotation file, and the corresponding eye tracking video. The annotations are then output in times relative to the eye tracking data for alignment. This can be seen in Figure \ref{fig:annotation}.

%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/annotation}
  \caption{Example output of the analysis tool parsing an annotation file. The time output represents the minutes, seconds, and milliseconds in the eye tracker video this annotation occurred. The annotations range from custom messages, or more standard messages like a new grasp set, change in task, or range point.}
  \label{fig:annotation}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%
---------Cindy has edited up to here


We check three things: how many people do we need, are the ranges we're getting valid, and can we successfully reconstruct the full 3D setup (object location wrt Barrett hand, eye tracking gaze location on 3D object)
To look for variation between human defined grasps we had four objects that were initially tested with three different subjects

[IMAGE - for 5 objects we tested on 3 people. Human grasp given, robot grasp given]

[TABLE - Similarity of grasp in terms of (normalized) variation of joint angles, number of finger contacts, palm/fingertip location with respect to object coordinate ] 

Plot of object with location variation as "blobs"

Table of average difference in position relative to bounding box size of object

\subsection{Validation of grasp ranges}

[IMAGE - for 5 objects show array of images with grasp extremes]

Using 3D location of object and hand, perform physical shake test in approximately same object orientation

5 shake tests per object at extreme of ranges

[TABLE - Object, person, grasp, success rate for plus and minus extreme]

% \subsection{Questionnaire}
% Answers to the post study questions

% \subsection{3D data reconstruction}
% \label {sec:PCArmCalibration}

% Image-based precision: Or 3D reconstruction, Barrett to kinect, glasses to kinect



==> temporal.tex <==
\subsection{Temporal calibration}
\label{sec:temporalCalibration}
% %%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
%   \centering
%   \includegraphics[width=0.8\linewidth]{images/enlarged_font_fftGraph}
%   \caption{An example plot of the Fast Fourier Transform return values used for beep detection. The program detects the first spike in the signal, and returns what time in the video the beep happened.}
%   \label{fig:fft}
%   \vspace{-0.1in}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%

The arm and Kinect data were timestamped and synced using a linux program called chrony running within ROS. The eye tracker, unfortunately, runs proprietary software on a stand-alone Windows laptop, so we used a 5 KhZ beep audio cue to mark a common point in both data streams. This beep is emitted from the ROS desktop machine using a key press at the beginning of data recording.

% We use a Fast Fourier transform to look for the 5 KhZ spike which was clearly seen in the eye tracker's audio stream (see Figure~\ref{fig:fft}). We search the audio stream in 100 ms windows, looking for a slope increase of 1, which produces an error around 50ms, worse case. 

